3D Pose Nowcasting: Forecast the Future to Improve the Present

Technologies to enable safe and effective collaboration and coexistence between humans and robots have gained significant importance in the last few years. A critical component useful for realizing this collaborative paradigm is the understanding of human and robot 3D poses using non-invasive systems. Therefore, in this paper, we propose a novel vision-based system leveraging depth data to accurately establish the 3D locations of skeleton joints. Specifically, we introduce the concept of Pose Nowcasting, denoting the capability of the proposed system to enhance its current pose estimation accuracy by jointly learning to forecast future poses. The experimental evaluation is conducted on two different datasets, providing accurate and real-time performance and confirming the validity of the proposed method on both the robotic and human scenarios.

==> tables/ablation.tex <==
\begin{table*}
    \begin{center}
    % \resizebox{1\linewidth}{!}{
    \begin{tabular}{l c l c ccccc c c}
    \toprule
        & & & & \multicolumn{5}{c}{\textbf{mAP} (\%) $\uparrow$} & & \\
        \cmidrule{5-9}
        \textbf{Input} & \textbf{Model} & \textbf{Timestep} & & $\mathbf{2}$cm & $\mathbf{4}$cm & $\mathbf{6}$cm & $\mathbf{8}$cm & $\mathbf{10}$cm & & \textbf{ADD} (cm) $\downarrow$ \\
        % \midrule
        % Depth + GT 3D joints & \textit{Ours} & $t$ & & $36.84$ & $69.58$ & $94.83$ & $99.60$ & $99.90$ & & $3.01 {\scriptstyle \, \pm 0.58}$ \\
        % Depth + GT 3D joints & \textit{Ours} & $t+0.5s$ & & $36.98$ & $69.17$ & $96.96$ & $99.38$ & $99.85$ & & $3.04 {\scriptstyle \, \pm 0.60}$ \\
        % Depth + GT 3D joints & \textit{Ours} & $t+1s$ & & $34.24$ & $62.76$ & $86.95$ & $93.17$ & $94.68$ & & $3.90 {\scriptstyle \, \pm 1.80}$ \\
        % Depth + GT 3D joints & \textit{Ours} & $t+1.5s$ & & $32.34$ & $59.19$ & $80.87$ & $88.20$ & $90.12$ & & $4.97 {\scriptstyle \, \pm 3.02}$ \\
        % Depth + GT 3D joints & \textit{Ours} & $t+2s$ & & $30.98$ & $56.47$ & $76.36$ & $83.54$ & $85.58$ & & $6.07 {\scriptstyle \, \pm 3.98}$ \\
        \midrule
        Depth + Pred. 3D joints & \textit{Ours} & $t$ & & $30.68$ & $66.90$ & $92.69$ & $98.02$ & $98.38$ & & $3.52 {\scriptstyle \, \pm 1.30}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+0.5s$ & & $31.32$ & $66.04$ & $91.71$ & $97.66$ & $98.33$ & & $3.57 {\scriptstyle \, \pm 1.33}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+1s$ & & $28.89$ & $59.67$ & $84.39$ & $91.04$ & $92.65$ & & $4.50 {\scriptstyle \, \pm 2.25}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+1.5s$ & & $26.41$ & $55.99$ & $78.14$ & $85.93$ & $87.93$ & & $5.71 {\scriptstyle \, \pm 3.48}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+2s$ & & $25.04$ & $53.43$ & $73.52$ & $81.27$ & $83.39$ & & $6.85 {\scriptstyle \, \pm 4.38}$ \\
        \midrule
        \textit{Ablation w/o temporal} \\
        \midrule
        Depth & \textit{Ours w/o temporal} & $t$ & & $11.06$ & $65.04$ & $95.41$ & $99.42$ & $99.75$ & & $3.60 {\scriptstyle \, \pm 0.75}$ \\
        Depth & \textit{Ours w/o temporal} & $t+0.5s$ & & $9.84$ & $63.80$ & $93.63$ & $99.04$ & $99.63$ & & $3.71 {\scriptstyle \, \pm 0.79}$ \\
        Depth & \textit{Ours w/o temporal} & $t+1s$ & & $9.47$ & $58.04$ & $86.59$ & $92.65$ & $94.23$ & & $4.61 {\scriptstyle \, \pm 1.90}$ \\
        Depth & \textit{Ours w/o temporal} & $t+1.5s$ & & $7.48$ & $52.67$ & $80.93$ & $87.54$ & $89.49$ & & $5.87 {\scriptstyle \, \pm 3.09}$ \\
        Depth & \textit{Ours w/o temporal} & $t+2s$ & & $7.14$ & $49.34$ & $75.53$ & $82.63$ & $84.69$ & & $7.15 {\scriptstyle \, \pm 4.06}$ \\
        \midrule
        \textit{Ablation w/o image} \\
        % \midrule
        % Depth + GT 3D joints & \textit{Ours} & $t$ & & $63.71$ & $94.32$ & $97.95$ & $99.18$ & $99.66$ & & $1.99 {\scriptstyle \, \pm 0.55}$ \\
        % Depth + GT 3D joints & \textit{Ours} & $t+0.5s$ & & $56.43$ & $88.13$ & $95.01$ & $98.41$ & $99.16$ & & $2.32 {\scriptstyle \, \pm 0.81}$ \\
        % Depth + GT 3D joints & \textit{Ours} & $t+1s$ & & $53.56$ & $82.40$ & $89.12$ & $93.03$ & $94.40$ & & $3.12 {\scriptstyle \, \pm 1.79}$ \\
        % Depth + GT 3D joints & \textit{Ours} & $t+1.5s$ & & $49.09$ & $79.13$ & $85.17$ & $89.24$ & $90.96$ & & $4.15 {\scriptstyle \, \pm 2.97}$ \\
        % Depth + GT 3D joints & \textit{Ours} & $t+2s$ & & $47.47$ & $76.25$ & $82.02$ & $86.15$ & $87.95$ & & $5.13 {\scriptstyle \, \pm 3.92}$ \\
        % \midrule
        % \midrule
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t$ & & $34.13$ & $68.39$ & $94.30$ & $99.57$ & $99.90$ & & $3.10 {\scriptstyle \, \pm 0.63}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+0.5s$ & & $33.45$ & $67.86$ & $93.44$ & $99.29$ & $99.83$ & & $3.15 {\scriptstyle \, \pm 0.68}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+1s$ & & $30.94$ & $61.11$ & $86.00$ & $92.72$ & $94.30$ & & $4.07 {\scriptstyle \, \pm 1.87}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+1.5s$ & & $28.27$ & $57.07$ & $79.49$ & $87.37$ & $89.54$ & & $5.22 {\scriptstyle \, \pm 3.08}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+2s$ & & $26.94$ & $54.35$ & $74.75$ & $82.50$ & $84.83$ & & $6.35 {\scriptstyle \, \pm 4.02}$ \\
        % \midrule

        % \textit{Ablation w/o temporal} \\
        % \midrule
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t$ & & $11.04$ & $64.69$ & $95.28$ & $99.4$ & $99.74$ & & $3.60 {\scriptstyle \, \pm 0.75}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+0.5s$ & & $9.84$ & $63.48$ & $93.50$ & $98.99$ & $99.61$ & & $3.71 {\scriptstyle \, \pm 0.79}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+1s$ & & $9.48$ & $57.47$ & $86.12$ & $92.31$ & $93.96$ & & $4.61 {\scriptstyle \, \pm 1.90}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+1.5s$ & & $7.45$ & $52.01$ & $80.31$ & $87.05$ & $89.09$ & & $5.87 {\scriptstyle \, \pm 3.09}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+2s$ & & $7.10$ & $48.54$ & $74.84$ & $82.02$ & $84.17$ & & $7.15 {\scriptstyle \, \pm 4.06}$ \\
        % \midrule

        % \textit{Ablation w/o image} \\
        % \midrule
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t$ & & $5.33$ & $22.77$ & $37.42$ & $57.96$ & $78.05$ & & $8.38 {\scriptstyle \, \pm 3.88}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+0.5s$ & & $4.77$ & $ 20.74$ & $37.31$ & $55.63$ & $76.53$ & & $ 8.61 {\scriptstyle \, \pm 4.07}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+1s$ & & $4.41$ & $19.65$ & $ 35.58$ & $53.16$ & $ 73.58$ & & $9.09 {\scriptstyle \, \pm 4.04}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+1.5s$ & & $4.12$ & $19.34$ & $33.40$ & $51.65$ & $72.08$ & & $9.73 {\scriptstyle \, \pm 4.23}$ \\
        % Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+2s$ & & $4.02$ & $18.81$ & $32.56$ & $ 50.32$ & $70.21$ & & $10.41 {\scriptstyle \, \pm 4.59}$ \\
        
        \midrule
        Pred. 3D joints & \textit{Ours w/o backbone} & $t$ & & $5.33$ & $22.77$ & $37.42$ & $57.96 & $78.05$ & & $8.38 {\scriptstyle \, \pm 3.88}$ \\
        Pred. 3D joints & \textit{Ours w/o backbone} & $t+0.5s$ & & $4.77$ & $20.74$ & $37.31$ & $55.63$ & $76.53$ & & $8.61 {\scriptstyle \, \pm 4.07}$ \\
        Pred. 3D joints & \textit{Ours w/o backbone} & $t+1s$ & & $4.41$ & $19.65$ & $35.58$ & $53.16$ & $73.58$ & & $ 9.09{\scriptstyle \, \pm 4.04}$ \\
        Pred. 3D joints & \textit{Ours w/o backbone} & $t+1.5s$ & & $4.12$ & $19.34$ & $33.40$ & $51.65$ & $72.08$ & & $ 9.73{\scriptstyle \, \pm 4.23}$ \\
        Pred. 3D joints & \textit{Ours w/o backbone} & $t+2s$ & & $4.02$ & $18.81$ & $32.56$ & $50.32$ & $70.21$ & & $ 10.41{\scriptstyle \, \pm 4.59}$ \\
        \bottomrule
    \end{tabular}
    % }
    \end{center}
    \caption{Ablation study on SimBa dataset choosing only one of the two inputs of the pipeline (the other is freezed to zero).}
    \label{tab:ablation-suppl}
\end{table*}

==> tables/itop_test.tex <==
\begin{table*}[t]
    \begin{center}
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l r c ccccc c c}
    \toprule
        & & \multicolumn{5}{c}{\textbf{mAP} (\%) $\uparrow$} & & \\
        \cmidrule{3-7}
        \textbf{Input} & \textbf{Method} & $\mathbf{2}$cm & $\mathbf{4}$cm & $\mathbf{6}$cm & $\mathbf{8}$cm & $\mathbf{10}$cm & & \textbf{ADD} (cm) $\downarrow$ \\
        \midrule
        Depth & RF~\cite{shotton2012efficient}  & $-$ & $-$ & $-$ & $-$ & $65.8$ & & $-$ \\
        Depth & IEF~\cite{carreira2016human}  & $-$ & $-$ & $-$ & $-$ & $71.0$ & & $-$ \\
        Depth & VI~\cite{haque2016towards}  & $-$ & $-$ & $-$ & $-$ & $77.4$ & & $-$ \\
        Depth & RTW~\cite{yub2015random}  & $-$ & $-$ & $-$ & $-$ & $80.5$ & & $-$ \\
        Depth & CMB~\cite{wang2018convolutional}  & $-$ & $-$ & $-$ & $-$ & $83.3$ & & $-$ \\
        Depth & REN$-$9x6x6~\cite{guo2017towards}  & $-$ & $-$ & $-$ & $-$ & $84.9$ & & $-$ \\
        Depth & A2J~\cite{xiong2019a2j}  & $-$ & $-$ & $-$ & $-$ & $88.0$ & & $-$ \\
        Voxelized Depth & V2V$^*$~\cite{moon2018v2v}  & $-$ & $-$ & $-$ & $-$ & $88.7$ & & $-$ \\
        Depth & DECA$-$D3~\cite{garau2021deca}  & $-$ & $-$ & $-$ & $-$ & $88.7$ & & $-$ \\
        Depth + PC & WSM~\cite{zhang2020weakly}  & $-$ & $-$ & $-$ & $-$ & $89.6$ & & $-$ \\
        Depth + PC & AdaPose~\cite{zhang2021sequential}  & $-$ & $-$ & $-$ & $-$ & $93.3$ & & $3.97$ \\
        \midrule
        Depth & \textit{Ours w/o forecasting} (vis.)  & $10.0$ & $38.6$ & $63.9$ & $79.2$ & $88.0$ & & $6.06$ \\
        Depth + Pred. 3D joints & \textit{Ours} (vis.)  & $11.0$ & $41.5$ & $68.5$ & $83.6$ & $90.6$ & & $5.71$ \\
        \midrule
        Depth & \textit{Ours w/o forecasting}  & $9.3$ & $36.1$ & $60.0$ & $75.1$ & $84.2$ & & $6.79$ \\
        Depth + Pred. 3D joints & \textit{Ours}  & $10.2$ & $38.8$ & $64.3$ & $79.1$ & $86.6$ & & $6.49$ \\
        \bottomrule
    \end{tabular}
    % }
    \end{center}
    \caption{Results on robot pose estimation on ITOP side-view test set. The proposed approach is evaluated in terms of mAP considering both visible and all joints. Method marked with $^*$ uses 10 models ensemble.}
    \label{tab:itop-3d-results}
\end{table*}

==> tables/itop_test_old.tex <==
\begin{table*}
    \begin{center}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l c c c ccccc c c}
    \toprule
        & & & & \multicolumn{5}{c}{\textbf{mAP} (\%) $\uparrow$} & & \\
        \cmidrule{5-9}
        \textbf{Input} & \textbf{Model} & \textbf{Time of prediction} & & $\mathbf{2}$cm & $\mathbf{4}$cm & $\mathbf{6}$cm & $\mathbf{8}$cm & $\mathbf{10}$cm & & \textbf{ADD} (cm) $\downarrow$ \\
        \midrule
        Image & RF~\cite{shotton2012efficient} & $t$ & & $-$ & $-$ & $-$ & $-$ & $65.80$ & & $-$ \\
        Image & IEF~\cite{carreira2016human} & $t$ & & $-$ & $-$ & $-$ & $-$ & $71.00$ & & $-$ \\
        Image & VI~\cite{haque2016towards} & $t$ & & $-$ & $-$ & $-$ & $-$ & $77.40$ & & $-$ \\
        Image & RTW~\cite{yub2015random} & $t$ & & $-$ & $-$ & $-$ & $-$ & $80.50$ & & $-$ \\
        % Image & RefineNet (D'Eusanio \etal 2020) & Curr & & $-$ & $-$ & $-$ & $-$ & $81.80$ & & $-$ \\
        Image & CMB~\cite{wang2018convolutional} & $t$ & & $-$ & $-$ & $-$ & $-$ & $83.30$ & & $-$ \\
        Image & REN$-$9x6x6~\cite{guo2017towards} & $t$ & & $-$ & $-$ & $-$ & $-$ & $84.90$ & & $-$ \\
        % Image & V3D (Pavllo \etal 2019) & Curr & & $-$ & $-$ & $-$ & $-$ & $87.69$ & & $-$ \\
        Image & A2J~\cite{xiong2019a2j} & $t$ & & $-$ & $-$ & $-$ & $-$ & $88.00$ & & $-$ \\
        Image & V2V$^*$~\cite{moon2018v2v} & $t$ & & $-$ & $-$ & $-$ & $-$ & $88.74$ & & $-$ \\
        Image & DECA$-$D3~\cite{garau2021deca} & $t$ & & $-$ & $-$ & $-$ & $-$ & $88.75$ & & $-$ \\
        Image & WSM~\cite{zhang2020weakly} & $t$ & & $-$ & $-$ & $-$ & $-$ & $89.59$ & & $-$ \\
        Image & AdaPose~\cite{zhang2021sequential} & $t$ & & $-$ & $-$ & $-$ & $-$ & $93.38$ & & $3.97$ \\
        \midrule
        3D joints & \textit{Last Points} & $t$ (vis. joints) & & $6.35$ & $13.80$ & $21.70$ & $29.46$ & $36.42$ & & $22.96$ \\
        3D joints & \textit{Last Points} & $t$ & & $5.87$ & $12.86$ & $20.28$ & $27.63$ & $34.26$ & & $24.33$ \\
        3D joints & \textit{Last Points} & $t+1$ & & $1.47$ & $6.15$ & $12.33$ & $19.63$ & $26.66$ & & $26.66$ \\
        3D joints & \textit{Linear} & $t$ (vis. joints) & & $14.65$ & $32.94$ & $46.94$ & $57.75$ & $66.42$ & & $10.24$ \\
        3D joints & \textit{Linear} & $t$ & & $13.59$ & $30.69$ & $44.05$ & $54.54$ & $63.18$ & & $11.30$ \\
        3D joints & \textit{Linear} & $t+1$ & & $0.77$ & $5.10$ & $13.16$ & $23.36$ & $33.16$ & & $20.06$ \\
        \midrule
        Image & \textit{Ours} (C) & $t$ (vis. joints) & & $10.03$ & $38.62$ & $63.86$ & $79.22$ & $87.96$ & & $6.06$ \\
        Image & \textit{Ours} (C) & $t$ & & $9.33$ & $36.10$ & $60.00$ & $75.06$ & $84.17$ & & $6.79$ \\
        \midrule
        % Image + 3D joints & SPDH (concat+Current+Future) & Curr & & $9.43$ & $35.55$ & $59.88$ & $74.27$ & $82.99$ & & $7.11$ \\
        % Image + 3D joints & SPDH (concat+Current+Future) & +1s & & $0.55$ & $3.69$ & $9.87$ & $17.47$ & $25.58$ & & $22.33$ \\
        Image + 3D joints & \textit{Ours} (C+F - 1s 1fps) & $t$ (vis. joints) & & $12.11$ & $43.91$ & $70.31$ & $84.20$ & $90.74$ & & $5.63$ \\
        Image + 3D joints & \textit{Ours} (C+F - 1s 1fps) & $t$ & & $11.25$ & $40.84$ & $65.85$ & $79.46$ & $86.51$ & & $6.44$ \\
        % Image + 3D joints & \textit{Ours} (C+F - 1s 1fps) & $t+1s$ (all frames) & & $0.65$ & $4.16$ & $10.94$ & $19.13$ & $27.81$ & & $21.56$ \\
        Image + 3D joints & \textit{Ours} (C+F - 1s 1fps) & $t+1$ & & $0.79$ & $4.72$ & $12.80$ & $22.59$ & $32.88$ & & $19.47$ \\
        \midrule
        Image + 3D joints & \textit{Ours} (C+F - 1s 2fps) & $t$ (vis. joints) & & $10.97$ & $41.53$ & $68.54$ & $83.62$ & $90.60$ & & $5.71$ \\
        Image + 3D joints & \textit{Ours} (C+F - 1s 2fps) & $t$ & & $10.19$ & $38.76$ & $64.32$ & $79.12$ & $86.57$ & & $6.49$ \\
        % Image + 3D joints & \textit{Ours} (C+F - 1s 2fps) & $t+0.5s$ (all frames) & & $1.75$ & $8.44$ & $18.48$ & $29.21$ & $38.74$ & & $19.33$ \\
        % Image + 3D joints & \textit{Ours} (C+F - 1s 2fps) & $t+1s$ (all frames) & & $0.97$ & $5.72$ & $13.43$ & $22.67$ & $31.62$ & & $21.11$ \\
        Image + 3D joints & \textit{Ours} (C+F - 1s 2fps) & $t+0.5$ & & $1.94$ & $9.61$ & $21.48$ & $33.91$ & $44.75$ & & $17.66$ \\
        Image + 3D joints & \textit{Ours} (C+F - 1s 2fps) & $t+1$ & & $1.20$ & $6.72$ & $16.39$ & $27.78$ & $38.56$ & & $18.94$ \\
        % \midrule
        % All Image & SPDH (double branch + upsampling) & Curr (all joints) & & $8.99$ & $35.44$ & $59.38$ & $74.20$ & $82.43$ & & $7.86$ \\
        % All Image & SPDH (double branch + upsampling) & Curr (visible joints) & & $$ & $$ & $$ & $$ & $86.39$ & & $6.98$ \\
        % \midrule
        % All Image + 3D joints & SPDH (concat+Current+Future) & Curr & & $6.69$ & $30.82$ & $55.47$ & $71.05$ & $80.60$ & & $8.18$ \\
        % All Image + 3D joints & SPDH (concat+Current+Future) & +1s & & $0.39$ & $2.65$ & $6.89$ & $12.35$ & $18.65$ & & $23.62$ \\
        % \midrule
        % All Image + 3D joints & SPDH (concat+Current+Future) & Curr & & $$ & $$ & $$ & $$ & $$ & & $$ \\
        % All Image + 3D joints & SPDH (concat+Current+Future) & +0.5s & & $$ & $$ & $$ & $$ & $$ & & $$ \\
        % All Image + 3D joints & SPDH (concat+Current+Future) & +1s & & $$ & $$ & $$ & $$ & $$ & & $$ \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{3D HPE and HPF results on ITOP side-view test sequences ( $^*$ indicates 10 models ensemble).}
    \label{tab:3d-results}
\end{table*}


\begin{table*}
    \begin{center}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l | ccccccccccc | cc}
    \toprule
         & \multicolumn{13}{c}{mAP (\%) at 10cm $\uparrow$} \\
        \midrule
         & & & & & & & & & & & & \textit{Ours} & \\
        \textbf{Joint} & RF~\cite{shotton2012efficient} & IEF~\cite{carreira2016human} & VI~\cite{haque2016towards} & RTW~\cite{yub2015random} & CMB~\cite{wang2018convolutional} & REN-9x6x6~\cite{guo2017towards} & A2J~\cite{xiong2019a2j} & V2V$^*$~\cite{moon2018v2v} & DECA-D3~\cite{garau2021deca} & WSM~\cite{zhang2020weakly} & AdaPose~\cite{zhang2021sequential} & \textit{w/o forecasting} & \textit{Ours} \\
        \midrule
        Head & $63.8$ & $96.2$ & $98.1$ & $97.8$ & $97.7$ & $98.7$ & $98.5$ & $98.3$ & $93.9$ & $98.1$ & $98.4$ & $98.2$ & $98.0$ \\
        Neck & $86.4$ & $85.2$ & $97.5$ & $95.8$ & $98.5$ & $99.4$ & $99.2$ & $99.1$ & $97.9$ & $99.5$ & $98.7$ & $98.7$ & $99.2$ \\
        Shoulders & $83.3$ & $77.2$ & $96.5$ & $94.1$ & $75.9$ & $96.1$ & $96.2$ & $97.2$ & $95.2$ & $94.7$ & $95.4$ & $96.7$ & $96.9$ \\
        Elbows & $73.2$ & $45.4$ & $73.3$ & $77.9$ & $62.7$ & $74.7$ & $78.9$ & $80.4$ & $84.5$ & $82.8$ & $90.7$ & $78.1$ & $78.1$ \\
        Hands & $51.3$ & $30.9$ & $68.7$ & $70.5$ & $84.4$ & $55.2$ & $68.3$ & $67.3$ & $56.5$ & $69.1$ & $82.1$ & $64.5$ & $64.8$ \\
        Torso & $65.0$ & $84.7$ & $85.6$ & $93.8$ & $96.0$ & $98.7$ & $98.5$ & $98.7$ & $99.0$ & $99.7$ & $99.7$ & $98.6$ & $98.6$ \\
        Hips & $50.8$ & $83.5$ & $72.0$ & $80.3$ & $87.9$ & $91.8$ & $90.8$ & $93.2$ & $97.4$ & $95.7$ & $96.4$ & $86.6$ &  $89.2$ \\
        Knees & $65.7$ & $81.8$ & $69.0$ & $68.8$ & $84.4$ & $89.0$ & $90.7$ & $91.8$ & $94.6$ & $91.0$ & $94.4$ & $84.8$ &  $87.8$ \\
        Feet & $61.3$ & $80.9$ & $60.8$ & $68.4$ & $83.8$ & $81.1$ & $86.9$ & $87.6$ & $92.0$ & $89.9$ & $92.8$ & $72.9$ &  $84.5$ \\
        \midrule
        Upper body & $70.7$ & $61.0$ & $84.0$ & $84.8$ & $80.6$ & $-$ & $-$ & $-$ & $83.0$ & $-$ & $-$ & $84.4$ & $84.6$ \\
        Lower body & $59.3$ & $82.1$ & $67.3$ & $72.5$ & $86.5$ & $-$ & $-$ & $-$ & $95.3$ & $-$ & $-$ & $83.8$ &  $88.8$ \\
        \midrule
        Total body & $65.8$ & $71.0$ & $77.4$ & $80.5$ & $83.4$ & $84.9$ & $88.0$ & $88.7$ & $88.7$ & $89.6$ & $93.4$ & $84.2$ &  $86.6$ \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{Per-joint results on robot pose estimation on ITOP side-view test set. Method marked with $^*$ uses 10 models ensemble.}
    \label{tab:3d-results}
\end{table*}

==> tables/simba_all_results.tex <==
\begin{table*}
    \begin{center}
    % \resizebox{1\linewidth}{!}{
    \begin{tabular}{l c l c ccccc c c}
    \toprule
        & & & & \multicolumn{5}{c}{\textbf{mAP} (\%) $\uparrow$} & & \\
        \cmidrule{5-9}
        \textbf{Input} & \textbf{Model} & \textbf{Timestep} & & $\mathbf{2}$cm & $\mathbf{4}$cm & $\mathbf{6}$cm & $\mathbf{8}$cm & $\mathbf{10}$cm & & \textbf{ADD} (cm) $\downarrow$ \\
        \midrule
        Depth + GT 3D joints & \textit{Ours} & $t$ & & $29.75$ & $69.11$ & $88.90$ & $98.26$ & $99.53$ & & $3.31 {\scriptstyle \, \pm 1.27}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+1s$ & & $26.64$ & $65.38$ & $88.31$ & $98.02$ & $99.30$ & & $3.50 {\scriptstyle \, \pm 1.22}$ \\
        \midrule
        Depth + GT 3D joints & \textit{Ours} & $t$ & & $28.34$ & $73.94$ & $92.43$ & $99.18$ & $99.60$ & & $3.18 {\scriptstyle \, \pm 1.00}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+1s$ & & $23.05$ & $68.74$ & $89.92$ & $98.91$ & $99.57$ & & $3.42 {\scriptstyle \, \pm 0.93}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+2s$ & & $20.50$ & $61.63$ & $80.06$ & $88.85$ & $90.89$ & & $5.22 {\scriptstyle \, \pm 3.11}$ \\
        \midrule
        Depth + GT 3D joints & \textit{Ours} & $t$ & & $24.48$ & $75.80$ & $97.02$ & $99.61$ & $99.91$ & & $3.04 {\scriptstyle \, \pm 0.65}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+0.5s$ & & $22.87$ & $74.42$ & $96.02$ & $99.19$ & $99.78$ & & $3.12 {\scriptstyle \, \pm 0.63}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+1s$ & & $22.89$ & $69.71$ & $89.20$ & $93.30$ & $94.89$ & & $3.88 {\scriptstyle \, \pm 1.78}$ \\
        \midrule
        Depth + GT 3D joints & \textit{Ours} & $t$ & & $36.84$ & $69.58$ & $94.83$ & $99.60$ & $99.90$ & & $3.01 {\scriptstyle \, \pm 0.58}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+0.5s$ & & $36.98$ & $69.17$ & $96.96$ & $99.38$ & $99.85$ & & $3.04 {\scriptstyle \, \pm 0.60}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+1s$ & & $34.24$ & $62.76$ & $86.95$ & $93.17$ & $94.68$ & & $3.90 {\scriptstyle \, \pm 1.80}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+1.5s$ & & $32.34$ & $59.19$ & $80.87$ & $88.20$ & $90.12$ & & $4.97 {\scriptstyle \, \pm 3.02}$ \\
        Depth + GT 3D joints & \textit{Ours} & $t+2s$ & & $30.98$ & $56.47$ & $76.36$ & $83.54$ & $85.58$ & & $6.07 {\scriptstyle \, \pm 3.98}$ \\
        \midrule
        \midrule
        Depth + Pred. 3D joints & \textit{Ours} & $t$ & & $27.77$ & $68.09$ & $88.58$ & $98.16$ & $99.50$ & & $3.40 {\scriptstyle \, \pm 1.25}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+1s$ & & $23.86$ & $63.13$ & $87.59$ & $97.77$ & $99.16$ & & $3.63 {\scriptstyle \, \pm 1.21}$ \\
        \midrule
        Depth + Pred. 3D joints & \textit{Ours} & $t$ & & $20.08$ & $64.70$ & $88.40$ & $98.47$ & $99.50$ & & $3.65 {\scriptstyle \, \pm 1.14}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+1s$ & & $17.20$ & $60.88$ & $85.95$ & $98.11$ & $99.42$ & & $3.86 {\scriptstyle \, \pm 1.07}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+2s$ & & $15.28$ & $53.37$ & $76.31$ & $87.53$ & $90.20$ & & $5.74 {\scriptstyle \, \pm 3.20}$ \\
        \midrule
        Depth + Pred. 3D joints & \textit{Ours} & $t$ & & $16.79$ & $61.68$ & $87.52$ & $92.49$ & $94.04$ & & $4.36 {\scriptstyle \, \pm 1.42}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+0.5s$ & & $14.97$ & $58.42$ & $84.47$ & $90.65$ & $93.43$ & & $4.57 {\scriptstyle \, \pm 1.43}$ \\
        Depth + Pred. 3D joints & \textit{Ours} & $t+1s$ & & $13.00$ & $52.53$ & $75.96$ & $83.66$ & $87.61$ & & $5.59 {\scriptstyle \, \pm 2.33}$ \\
        \midrule
        \midrule
        Pred. 3D joints & \textit{Linear} & $t$ & & $0.31$ & $6.02$ & $15.81$ & $25.78$ & $41.23$ & & $ 16.89{\scriptstyle \, \pm  5.73}$ \\
        Pred. 3D joints & \textit{Linear} & $t+0.5s$ & & $0.42$ & $5.54$ & $15.34$ & $25.40$ & $40.58$ & & $ 17.54 {\scriptstyle \, \pm 6.20}$ \\
        Pred. 3D joints & \textit{Linear} & $t+1s$ & & $0.29$ & $4.78$ & $14.76$ & $23.44$ & $38.08$ & & $19.25 {\scriptstyle \, \pm 6.20}$ \\
        Pred. 3D joints & \textit{Linear} & $t+1.5s$ & & $0.32$ & $4.34$ & $14.11$ & $22.76$ & $36.72$ & & $19.75 {\scriptstyle \, \pm 6.17}$ \\
        Pred. 3D joints & \textit{Linear} & $t+2s$ & & $0.37$ & $3.98$ & $13.72$ & $21.84$ & $35.96$ & & $ 20.04{\scriptstyle \, \pm 6.10}$ \\
        \midrule
        Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t$ & & $34.13$ & $68.39$ & $94.30$ & $99.57$ & $99.90$ & & $3.10 {\scriptstyle \, \pm 0.63}$ \\
        Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+0.5s$ & & $33.45$ & $67.86$ & $93.44$ & $99.29$ & $99.83$ & & $3.15 {\scriptstyle \, \pm 0.68}$ \\
        Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+1s$ & & $30.94$ & $61.11$ & $86.00$ & $92.72$ & $94.30$ & & $4.07 {\scriptstyle \, \pm 1.87}$ \\
        Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+1.5s$ & & $28.27$ & $57.07$ & $79.49$ & $87.37$ & $89.54$ & & $5.22 {\scriptstyle \, \pm 3.08}$ \\
        Depth + Pred. 3D joints (Baseline) & \textit{Ours} & $t+2s$ & & $26.94$ & $54.35$ & $74.75$ & $82.50$ & $84.83$ & & $6.35 {\scriptstyle \, \pm 4.02}$ \\
        \midrule
        Depth + Pred. 3D joints (\textcolor{red}{Ours}) & \textit{Ours} & $t$ & & $30.68$ & $66.90$ & $92.69$ & $98.02$ & $98.38$ & & $3.52 {\scriptstyle \, \pm 1.30}$ \\
        Depth + Pred. 3D joints (\textcolor{red}{Ours}) & \textit{Ours} & $t+0.5s$ & & $31.32$ & $66.04$ & $91.71$ & $97.66$ & $98.33$ & & $3.57 {\scriptstyle \, \pm 1.33}$ \\
        Depth + Pred. 3D joints (\textcolor{red}{Ours}) & \textit{Ours} & $t+1s$ & & $28.89$ & $59.67$ & $84.39$ & $91.04$ & $92.65$ & & $4.50 {\scriptstyle \, \pm 2.25}$ \\
        Depth + Pred. 3D joints (\textcolor{red}{Ours}) & \textit{Ours} & $t+1.5s$ & & $26.41$ & $55.99$ & $78.14$ & $85.93$ & $87.93$ & & $5.71 {\scriptstyle \, \pm 3.48}$ \\
        Depth + Pred. 3D joints (\textcolor{red}{Ours}) & \textit{Ours} & $t+2s$ & & $25.04$ & $53.43$ & $73.52$ & $81.27$ & $83.39$ & & $6.85 {\scriptstyle \, \pm 4.38}$ \\
        \midrule
        Depth + Pred. 3D joints (\textcolor{green}{Ours 16bit}) & \textit{Ours} & $t$ & & $27.64$ & $59.27$ & $85.20$ & $90.95$ & $91.69$ & & $6.51 {\scriptstyle \, \pm 5.50}$ \\
        Depth + Pred. 3D joints (\textcolor{green}{Ours 16bit}) & \textit{Ours} & $t+0.5s$ & & $26.26$ & $59.09$ & $84.62$ & $90.81$ & $91.61$ & & $6.95 {\scriptstyle \, \pm 6.56}$ \\
        Depth + Pred. 3D joints (\textcolor{green}{Ours 16bit}) & \textit{Ours} & $t+1s$ & & $23.88$ & $53.16$ & $77.65$ & $84.26$ & $85.98$ & & $7.85 {\scriptstyle \, \pm 6.82}$ \\
        Depth + Pred. 3D joints (\textcolor{green}{Ours 16bit}) & \textit{Ours} & $t+1.5s$ & & $21.58$ & $49.88$ & $71.87$ & $79.50$ & $81.49$ & & $9.16 {\scriptstyle \, \pm 7.79}$ \\
        Depth + Pred. 3D joints (\textcolor{green}{Ours 16bit}) & \textit{Ours} & $t+2s$ & & $20.62$ & $47.53$ & $67.64$ & $75.03$ & $77.11$ & & $10.26 {\scriptstyle \, \pm 8.10}$ \\
        \midrule
        Depth + Pred. 3D joints (\textcolor{green}{Ours 32bit}) & \textit{Ours} & $t$ & & $27.67$ & $59.23$ & $85.18$ & $90.96$ & $91.68$ & & $6.50 {\scriptstyle \, \pm 5.14}$ \\
        Depth + Pred. 3D joints (\textcolor{green}{Ours 32bit}) & \textit{Ours} & $t+0.5s$ & & $26.34$ & $59.03$ & $84.55$ & $90.88$ & $91.64$ & & $6.98 {\scriptstyle \, \pm 6.44}$ \\
        Depth + Pred. 3D joints (\textcolor{green}{Ours 32bit}) & \textit{Ours} & $t+1s$ & & $23.87$ & $53.10$ & $77.54$ & $84.25$ & $85.94$ & & $7.93 {\scriptstyle \, \pm 6.85}$ \\
        Depth + Pred. 3D joints (\textcolor{green}{Ours 32bit}) & \textit{Ours} & $t+1.5s$ & & $21.58$ & $49.88$ & $71.78$ & $79.48$ & $81.50$ & & $9.22 {\scriptstyle \, \pm 7.72}$ \\
        Depth + Pred. 3D joints (\textcolor{green}{Ours 32bit}) & \textit{Ours} & $t+2s$ & & $20.59$ & $47.52$ & $67.58$ & $75.01$ & $77.08$ & & $10.34 {\scriptstyle \, \pm 8.10}$ \\
        % \midrule
        % Pred. 3D joints & \textit{Copy last} & $t$ & & $2.72$ & $21.95$ & $34.54$ & $47.86$ & $71.34$ & & $10.93 {\scriptstyle \, \pm 5.36}$ \\
        % Pred. 3D joints & \textit{Copy last} & $t+0.5$ & & $$ & $$ & $$ & $$ & $$ & & ${\scriptstyle \, \pm }$ \\
        % Pred. 3D joints & \textit{Copy last} & $t+1$ & & $$ & $$ & $$ & $$ & $$ & & $ {\scriptstyle \, \pm }$ \\
        % Pred. 3D joints & \textit{Copy last} & $t+1.5$ & & $$ & $$ & $$ & $$ & $$ & & $ {\scriptstyle \, \pm }$ \\
        % Pred. 3D joints & \textit{Copy last} & $t+2$ & & $$ & $$ & $$ & $$ & $$ & & $ {\scriptstyle \, \pm }$ \\
        \bottomrule
    \end{tabular}
    % }
    \end{center}
    \caption{Results on both robot pose estimation and forecasting on SimBa dataset. The proposed method is compared to a linear model while tested in an autoregressive manner, taking as input the predicted 3D pose of the past $T$ frames.}
    \label{tab:simba-all-results}
\end{table*}

% Last point and Linear with gt joints
% 3D Joints & \textit{Last point} & $t$ & & $82.62$ & $86.47$ & $89.1$ & $90.7$ & $91.86$ & & $ 2.32{\scriptstyle \, \pm 3.05}$ \\
% 3D Joints & \textit{Last point} & $t+1$ & & $82.11$ & $85.9$ & $88.47$ & $90.22$ & $91.43$ & & $ 2.47{\scriptstyle \, \pm 3.20}$ \\
% 3D Joints & \textit{Last point} & $t+2$ & & $75.38$ & $79.06$ & $81.74$ & $83.87$ & $85.60$ & & $ 4.64{\scriptstyle \, \pm 4.87}$ \\
% 3D Joints & \textit{Linear} & $t$ & & $96.92$ & $99.57$ & $99.96$ & $100.0 $ & $100.0 $ & & $0.29 {\scriptstyle \, \pm 0.28}$ \\
% 3D Joints & \textit{Linear} & $t+1$ & & $94.03$ & $97.86$ & $99.37$ & $99.81$ & $99.96$ & & $0.55 {\scriptstyle \, \pm 0.45}$ \\
% 3D Joints & \textit{Linear} & $t+2$ & & $80.80$ & $85.37$ & $87.96$ & $90.01$ & $91.45$ & & $3.10 {\scriptstyle \, \pm 3.00}$ \\

% Ours (2s 1fps) with Pred.iction at 10fps with supervision on 1 and 2 second
% Depth + 3D joints & SPDH (concat+Current+Future) & Curr & & $18.15$ & $65.05$ & $90.73$ & $98.10$ & $99.40$ & & $3.68 {\scriptstyle \, \pm 0.81}$ \\
% Depth + 3D joints & SPDH (concat+Current+Future) & +1s & & $$ & $$ & $$ & $$ & $$ & & $5.48 {\scriptstyle \, \pm 2.87}$ \\
% Depth + 3D joints & SPDH (concat+Current+Future) & +2s & & $$ & $$ & $$ & $$ & $$ & & $8.25 {\scriptstyle \, \pm 4.54}$ \\

% Ours (2s 1fps) with deltas
% Depth + 3D joints & SPDH (concat+Current+Future) & Curr & & $16.70$ & $60.30$ & $92.29$ & $99.41$ & $99.88$ & & $3.65 {\scriptstyle \, \pm 0.63}$ \\
% Depth + 3D joints & SPDH (concat+Current+Future) & +1s & & $16.22$ & $58.11$ & $92.87$ & $99.04$ & $99.79$ & & $3.70 {\scriptstyle \, \pm 0.69}$ \\
% Depth + 3D joints & SPDH (concat+Current+Future) & +2s & & $14.99$ & $50.62$ & $81.96$ & $88.79$ & $90.88$ & & $5.50 {\scriptstyle \, \pm 3.09}$ \\

==> tables/single-arm-movements.tex <==
\begin{table*}
    \begin{center}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{ll c c c ccccc c c}
    \toprule
        & & & & & \multicolumn{5}{c}{\textbf{mAP} (\%) $\uparrow$} & & \\
        \cmidrule{6-10}
        \textbf{Method} & \textbf{Input} & \textbf{Features} & \textbf{Aggreg.} & & $\mathbf{2}$cm & $\mathbf{4}$cm & $\mathbf{6}$cm & $\mathbf{8}$cm & $\mathbf{10}$cm & & \textbf{ADD} (cm) $\downarrow$ \\
        \midrule
        SPDH & Img & Visual & & & $6.33$ & $53.75$ & $79.75$ & $93.90$ & $98.12$ &  & $4.41 {\scriptstyle \, \pm 1.09}$ \\
        SPDH & Img & Visual & & & $$ & $$ & $$ & $$ & $$ &  & $ {\scriptstyle \, \pm }$ \\
        
        \midrule
        D-SPDH ups. & Img & Vis. & & & $15.30$ & $54.68$ & $88.12$ & $98.13$ & $99.44$ & & $4.01 {\scriptstyle \, \pm 0.59}$ \\
        \midrule
        D-SPDH ups. & Img & Vis. + Random & Concat & & $12.71$ & $56.60$ & $87.19$ & $98.62$ & $99.52$ &  & $3.92 {\scriptstyle \, \pm 0.80}$ \\
        -- & 3D & last prev joints & 3D & & $97.64 $ & $99.88 $ & $99.99 $ & $100.0 $ & $100.0$ &  & $0.17 {\scriptstyle \, \pm 0.24}$\\
        \midrule
        D-SPDH ups. & Img + Displ. & Vis. + Local GRU & Concat & & $8.88$ & $51.41$ & $81.62$ & $95.64$ & $99.29$ &  & $ 4.37{\scriptstyle \, \pm 0.86} $ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local GRU & Concat & & $7.74$ & $49.56$ & $84.15$ & $98.61$ & $99.54$ &  & $ 4.22 {\scriptstyle \, \pm  0.56}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Global GRU & Concat & & $15.04$ & $59.10$ & $90.73$ & $98.70$ & $99.65$ &  & $ 3.76{\scriptstyle \, \pm 0.89}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local/Global GRU & Concat & & $4.54$ & $ 48.60$ & $75.26$ & $85.87$ & $92.53$ &  & $ 5.25{\scriptstyle \, \pm 1.09}$ \\
        \midrule
        D-SPDH ups. & Img + Displ. & Vis. + Local GRU & Cross-Attn (temp2vis) & & $6.68$ & $45.37$ & $89.40$ & $93.49$ & $94.47$ &  & $4.76 {\scriptstyle \, \pm 1.15}$ \\
        D-SPDH ups. & Img + Displ. & Vis. + Local GRU & Cross-Attn (vis2temp) & & $14.86$ & $53.29$ & $88.60$ & $96.57$ & $97.45$ &  & $4.08 {\scriptstyle \, \pm 1.56}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local GRU & Cross-Attn (temp2vis) & & $4.10$ & $28.19$ & $67.86$ & $92.08$ & $98.64$ &  & $5.18 {\scriptstyle \, \pm 0.80}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local GRU & Cross-Attn (vis2temp) & & $0.98$ & $3.14$ & $8.39$ & $12.14$ & $20.74$ &  & $18.69 {\scriptstyle \, \pm 3.13}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Global GRU & Cross-Attn (temp2vis) & & $13.65$ & $50.30$ & $74.20$ & $92.97$ & $98.78$ &  & $4.49 {\scriptstyle \, \pm 0.79}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Global GRU & Cross-Attn (vis2temp) & & $11.88$ & $50.00$ & $77.75$ & $92.91$ & $96.48$ &  & $4.50 {\scriptstyle \, \pm 0.65}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local/Global GRU & Cross-Attn (temp2vis) & & $10.79$ & $51.90$ & $87.48$ & $98.48$ & $99.38$ &  & $4.12 {\scriptstyle \, \pm 0.58}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local/Global GRU & Cross-Attn (vis2temp) & & $0.00$ & $1.99$ & $7.56$ & $14.29$ & $21.49$ &  & $18.97 {\scriptstyle \, \pm 4.13}$ \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{3D RPE results on SimBa$^{++}$ real sequences with single-arm movements}
    \label{tab:3d-results}
\end{table*}

==> tables/synth_results.tex <==
% \begin{sidewaystable*}
\begin{table*}
    \begin{center}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{ll c c c ccccc c c}
    \toprule
        & & & & & \multicolumn{5}{c}{\textbf{mAP} (\%) $\uparrow$} & & \\
        \cmidrule{6-10}
        \textbf{Method} & \textbf{Input} & \textbf{Features} & \textbf{Aggreg.} & & $\mathbf{2}$cm & $\mathbf{4}$cm & $\mathbf{6}$cm & $\mathbf{8}$cm & $\mathbf{10}$cm & & \textbf{ADD} (cm) $\downarrow$ \\        
        \midrule
        D-SPDH ups. & Img & Vis. & & & $95.96$ & $99.37$ & $99.89$ & $99.96$ & $99.98$ &  & $0.93 {\scriptstyle \, \pm 0.32}$ \\
        \midrule
        D-SPDH ups. & Img & Vis. + Random & Concat & & $95.35$ & $99.60$ & $99.9$ & $9.96$ & $99.97$ &  & $0.94 {\scriptstyle \, \pm 0.60}$ \\
        
        \midrule
        D-SPDH ups. & Img + Displ. & Vis. + Local GRU & Concat & & $96.87$ & $99.63$ & $99.9$ & $99.95$ & $99.97$ &  & $ 0.87 {\scriptstyle \, \pm 0.29}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local GRU & Concat & & $91.34$ & $99.73$ & $99.93$ & $99.93$ & $ 99.96$ &  & $ 1.07 {\scriptstyle \, \pm 0.46}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Global GRU & Concat & & $96.89$ & $99.61$ & $99.92$ & $99.96$ & $99.97 $ &  & $ 0.90 {\scriptstyle \, \pm 0.28}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local/Global GRU & Concat & & $97.43$ & $99.81$ & $99.94$ & $99.96$ & $99.98$ &  & $ 0.87 {\scriptstyle \, \pm 0.26}$ \\
        \midrule
        D-SPDH ups. & Img + Displ. & Vis. + Local GRU & Cross-Attn (temp2vis) & & $97.20$ & $99.77$ & $99.94$ & $99.97$ & $99.98$ &  & $0.89 {\scriptstyle \, \pm 0.23}$ \\
        D-SPDH ups. & Img + Displ. & Vis. + Local GRU & Cross-Attn (vis2temp) & & $91.14$ & $99.23$ & $99.85$ & $99.93$ & $99.95$ &  & $1.08 {\scriptstyle \, \pm 0.62}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local GRU & Cross-Attn (temp2vis) & & $96.78$ & $99.71$ & $99.95$ & $99.98$ & $99.98$ &  & $0.91 {\scriptstyle \, \pm 0.26}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local GRU & Cross-Attn (vis2temp) & & $23.74$ & $55.25$ & $69.98$ & $78.52$ & $84.45$ &  & $6.11 {\scriptstyle \, \pm 3.95}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Global GRU & Cross-Attn (temp2vis) & & $95.74$ & $99.56$ & $99.93$ & $99.97$ & $99.98$ &  & $0.96 {\scriptstyle \, \pm 0.31}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Global GRU & Cross-Attn (vis2temp) & & $95.73$ & $99.59$ & $99.94$ & $99.98$ & $99.98$ &  & $0.93 {\scriptstyle \, \pm 0.29}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local/Global GRU & Cross-Attn (temp2vis) & & $95.49$ & $99.59$ & $99.93$ & $99.96$ & $99.97$ &  & $0.93 {\scriptstyle \, \pm 0.32}$ \\
        D-SPDH ups. & Img + Absolute & Vis. + Local/Global GRU & Cross-Attn (vis2temp) & & $25.11$ & $56.11$ & $70.28$ & $79.37$ & $85.62$ &  & $5.56 {\scriptstyle \, \pm 3.70}$ \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{3D RPE results on SimBa$^{++}$ synthetic sequences}
    \label{tab:3d-results}
\end{table*}
% \end{sidewaystable*}
